Arbitrarily Fast Multivariable Least-squares MRAC

A novel least-squares model-reference direct adaptive control (LS-MRAC) algorithm for multivariable (MIMO) plants is presented. The controller parameters are directly updated based on the output tracking error. The control law is crucially modified to reduce the relative degree of the error model to zero. A complete Lyapunov-based stability analysis as well as a tracking error convergence characterization is provided demonstrating that the LS-MRAC can achieve arbitrarily fast tracking while maintaining satisfactory parameter convergence for appropriate adaptation gains. Simulation results show a significant improvement in tracking performance compared to previous methods.

==> formato.tex <==
% Formato IEEE R&A
% Muda o estilo da letra nas seções e subseções

\makeatletter
\def\@normalsize{\@setsize\normalsize{10pt}\xpt\@xpt
  \abovedisplayskip 10pt plus2pt minus5pt\belowdisplayskip \abovedisplayskip
  \abovedisplayshortskip \z@ plus3pt\belowdisplayshortskip 6pt plus3pt
   minus3pt\let\@listi\@listI}

\def\subsize{\@setsize\subsize{12pt}\xipt\@xipt}
\def\section{\@startsection {section}{1}{\z@}{1.0ex plus 1ex minus .2ex}
						{.2ex plus .2ex}{\large\bf}}

\def\subsection{\@startsection {subsection}{2}{\z@}{.2ex plus 1ex}{.2ex plus .2ex}
						{\subsize\bf}}
\makeatother

